Finding k-Dissimilar Paths with Minimum Collective Length

Shortest path computation is a fundamental problem in road networks. However, in many real-world scenarios, determining solely the shortest path is not enough. In this paper, we study the problem of finding k-Dissimilar Paths with Minimum Collective Length (kDPwML), which aims at computing a set of paths from a source s to a target t such that all paths are pairwise dissimilar by at least \theta and the sum of the path lengths is minimal. We introduce an exact algorithm for the kDPwML problem, which iterates over all possible s-t paths while employing two pruning techniques to reduce the prohibitively expensive computational cost. To achieve scalability, we also define the much smaller set of the simple single-via paths, and we adapt two algorithms for kDPwML queries to iterate over this set. Our experimental analysis on real road networks shows that iterating over all paths is impractical, while iterating over the set of simple single-via paths can lead to scalable solutions with only a small trade-off in the quality of the results.

==> chapters/kspd.tex <==
\section{$K$-Shortest Paths with Diversity} \label{sec:kspd}

\nr{
See MPUP for what to write
% To the best of our knowledge, the problem of finding Top-$k$ Shortest Paths with Diversity
% ($\mathit{Top{-}KSPD}$) introduced by Liu at al.~\cite{liu2017} is the most similar work to
% our own. However, despite introducing the \kdsp problem, the authors do not propose an exact
% algorithm, but only a greedy heuristic evaluation of $\mathit{Top{-}KSPD}$ queries.
% First, the shortest path is added to the result set $P$. Next, paths are examined in ascending
% order of their length. When an alternative path to $P$ is found, it is added to the result set.
% The algorithm continues examining paths until either $k$ paths have been added to the result
% set or there are no more paths left to examine. 
% More specifically, the authors build upon the computation of the $K$-shortest simple
% paths (\ksp)~\cite{hershberger2007,martins2003,yen1971} and propose a routine for computing
% the next shortest path in length order. The proposed routine employs a path classification
% scheme, similar to the one proposed by Hershberger at al.~\cite{hershberger2007} for the
% same purpose. To compute the \kdsp, the authors first propose a baseline algorithm
% $\mathit{ApproximateKSPD}$ which examines paths in length order, and subsequently introduce
% the $\mathit{FindKSPD}$ algorithm which employs their \ksp routine along with a path
% similarity-based lower bound in order to reduce the number of paths that need to be constructed.
% We model alternative routing as the problem of finding
% \emph{Top-$k$ Shortest Paths with Diversity} (\kdsp);
% More formally:
}

\begin{problem}[\kdsp]
Given a road network $G = (N,E)$, a source and a target node $s, t \in N$, a number of requested paths $k$, 
and a similarity threshold $\theta$, find a set of paths \PDSP from $s$ to $t$, such that:
\begin{enumerate}
\item $\forall p \in \PDSP$, $p$ is an alternative path to set $\PDSP \setminus \{p\}$ w.r.t. threshold $\theta$,
\item $\vert \PDSP \vert \leq k$ and $\not\exists \PDSPP : \vert \PDSP \vert < \vert \PDSPP \vert$ which satisfies bullet (1), and
\item \PDSP has the lowest collective path length among all sets
  $P_{alt}$ of $k$ paths from $s$ to $t$, which satisfy Condition (1),
  i.e.,
\[
%\PDSP = \arg \min_{P_{alt}} \sum\limits_{\forall p \in P_{alt}}{\ell(p)}
\PDSP = \arg \min_{P_{alt}} \LEN(P_{alt}).
\]
\end{enumerate}
\label{def:kdsp}
\end{problem}

\tc{Clarify the problem definition here.}

\tc{If we add the proof of complexity, we need to say why we do it as the TKDE paper already provided a proof
on the NP-hardness. Maybe we can support our proof by saying something like "although the authors have shown
that the problem is NP-hard, we show that the problem is strongly NP-hard" and elaborate a bit on that.}
Next, we elaborate on the complexity of the \kdsp problem.
%
\begin{theorem}
The \kdsp problem is strongly $NP$-hard.
\end{theorem}
\begin{proof}
We prove the lemma by reduction from the two edge-disjoint path problem in directed
graphs ($2$-DP), which is known to be strongly
$NP$-complete~\cite{fortune1980,eilam-tzoreff1998}. Given a directed graph
$G=(N,E)$ and two source-target pairs $(s_1,t_1)$ and $(s_2,t_2)$, $2$-DP asks to
correctly decide if $G$ contains edge-disjoint $(s_i{\rightarrow}t_i)$ paths for $i=1,2$.
Reducing $2$-DP to the task of answering \kdsp queries with $k=2$ is straightforward:
we define a road network $G^\prime=(N^\prime,E^\prime)$ with $N^\prime=N\cup\{s,t\}$ and
$E^\prime=E\cup\{(s,s_1),(s,s_2),(t_1,t),(t_2,t)\}$, define $\ell(e)=0$ for
all $e\in E^\prime$, and set $\theta=0$. Then there are edge-disjoint $(s_i{\rightarrow}t_i)$-paths
in $G$ just in case the result of a $2$-DPwML query against $G^\prime$ is not the empty
set. Therefore, unless $P=NP$, there can be no polynomial or pseudo-polynomial algorithm
for answering \kdsp queries.
\end{proof}

\tc{Originally we used this example to show that there is not way to have guarantees for the
greedy approximation. However, we can use the same example to additionally emphasize the
shortcoming of the greedy approach, i.e., that it is always possible to not find $k$ results
even if they exist. That will motivate our idea to examine combinations which exclude the shortest path.}
\nr{
Despite the good results, there can be no theoretical bound for the collective path length; in other words,
the cummulative length of the result set of the greedy approach $\PGREEDY$ can be arbitrarily higher than the optimal one.
To elaborate, consider Figure~\ref{fig:no-approx-possible}, which shows
four paths from $s$ to $t$: $\sp = \langle (s,n_1),(n_1,n_2),(n_2,t) \rangle$ with $\len(p_1) = 3a$,
$p_2 = \langle (s,n_1),(n_1,u_1),(u_1,t) \rangle$ with $\len(p_2) = 5a$,
$p_3 = \langle (s,u_2),(u_2,n_2),(n_2,t) \rangle$ with $\len(p_3) = 5a$, and
$p_4 = \langle (s,\ldots),\ldots,(\ldots,t) \rangle$ with $\len(p_4) = m$.  Let $m$ be arbitrarily
larger than $a$ such that $p_4$ is always the longest path. For $k=3$ and $\theta = 0\%$, the result
of \kdsp is $\PDSP = \{p_2,p_3\}$ with $\LEN(\PDSP) = 10a$. In contrast, 
$\PGREEDY = \{p_1,p_4\}$ with $\LEN(\PGREEDY) = 3 + m$ (as the shortest path $\sp \in \PGREEDY$, $p_2$ and $p_3$
are excluded for being too similar to $p_1$).  Since $m$ can be arbitrarily large, there is no upper
bound for $\LEN(\PGREEDY)$.
}
\begin{figure}[htb]
\begin{tikzpicture}[
		auto,
		node distance=1cm,
 		thick,
  		point/.style={
  			circle,
  			draw,
  			font=\scriptsize,
  			fill=white,
  			minimum size = 14pt,
  			inner sep=0pt
  		},
  		myline/.style={
  			line width=0.5pt,
  			every node/.style={font=\scriptsize},
  			color=black
  		},
	]
	\input{tikz/noapprox.tikz}
\end{tikzpicture}
%\caption{Road network demonstrating that no approximation bound is possible.}
\caption{Example for the lack of upper bound on $\LEN(\PGREEDY)$.}
\label{fig:no-approx-possible}
\end{figure}


==> tables/completeness-scalable.tex <==
\def\arraystretch{0.9}
\begin{tabular}{|c|r||c|c|}
  \hline
  %\textbf{Road network} 
  \cellcolor{gray!60}Road network
  & \cellcolor{gray!60}$k$
  & \cellcolor{gray!60}\svpplus
  & \cellcolor{gray!60}\esx
  \\\hline\hline
  \multirow{4}{*}{Milan}
& 4		&	100 	&	99.4		\\
& 8		&	99.5 	&	97.4	\\
& 12	&	98.0 	&	95.2		\\
& 16	&	90.2 	&	94.2	\\
		\hline
		\multirow{4}{*}{Chicago}
& 4		&	100 	&	99.3		\\
& 8		&	100 	&	96.6		\\
& 12	&	99.4 	&	94.4	\\
& 16	&	97.7 	&	93.1	\\
		\hline
		\multirow{4}{*}{Colorado}
& 4		&	99.8 	&	98.9	\\
& 8 	&	91.2	&	97.5	\\
& 12	&	62.5 	&	96.0	\\
& 16 	&	38.1	&	95.2	\\
		\hline
		\multirow{4}{*}{Florida}
& 4 	&	98.7	&	99.3	\\
& 8 	&	75.0	&	98.0	\\
& 12 	&	39.5	&	97.5	\\
& 16 	&	7.4		&	96.9	\\
		\hline
\end{tabular}

